DINO-X: A Unified Vision Model for Open-World Object Detection and Understanding

In this paper, we introduce DINO-X, which is a unified object-centric vision model developed by IDEA Research with the best open-world object detection performance to date. DINO-X employs the same Transformer-based encoder-decoder architecture as Grounding DINO 1.5 to pursue an object-level representation for open-world object understanding. To make long-tailed object detection easy, DINO-X extends its input options to support text prompt, visual prompt, and customized prompt. With such flexible prompt options, we develop a universal object prompt to support prompt-free open-world detection, making it possible to detect anything in an image without requiring users to provide any prompt. To enhance the model's core grounding capability, we have constructed a large-scale dataset with over 100 million high-quality grounding samples, referred to as Grounding-100M, for advancing the model's open-vocabulary detection performance. Pre-training on such a large-scale grounding dataset leads to a foundational object-level representation, which enables DINO-X to integrate multiple perception heads to simultaneously support multiple object perception and understanding tasks, including detection, segmentation, pose estimation, object captioning, object-based QA, etc. Experimental results demonstrate the superior performance of DINO-X. Specifically, the DINO-X Pro model achieves 56.0 AP, 59.8 AP, and 52.4 AP on the COCO, LVIS-minival, and LVIS-val zero-shot object detection benchmarks, respectively. Notably, it scores 63.3 AP and 56.5 AP on the rare classes of LVIS-minival and LVIS-val benchmarks, improving the previous SOTA performance by 5.8 AP and 5.0 AP. Such a result underscores its significantly improved capacity for recognizing long-tailed objects.

==> sec/caption.tex <==
We developed a unified, task-promotable text decoder to enhance DINO-X's ability to comprehend regional context and perform perception tasks beyond localization, such as referring object classification, region captioning, text recognition, and region-based visual question answering (VQA). The architecture of our model is depicted in Figure \ref{fig:dinox_cap}. Initially, we utilize a frozen DINO-X to extract object tokens for region representation from the input image. Specifically, we derive region features from backbone features using the RoIAlign \cite{he2017mask} operator, combined with query embeddings to form our object tokens. Then, we apply a simple linear projection to ensure their dimensions aligned with the text embedding. The lightweight text decoder integrates these regional representations with task tokens to generate outputs in an auto-regressive manner. The learnable task tokens empower the text decoder to handle a variety of tasks.



%\begin{figure}[ht!]
%\centering
% \includegraphics[width=0.75\textwidth,keepaspectratio]{figs/dino_x_caption_head.pdf}
% \caption{The detailed design of text decoder in DINO-X. It involves using a frozen DINO-X to extract object tokens, and a linear projection aligns its dimensions with the text embeddings. The lightweight text decoder then integrates these object and task tokens to generate response outputs in an autoregressive manner. The task tokens equip the text decoder with the capability of tackling different tasks.}
% \label{fig:dinox_cap}
%\end{figure}

%
%It consists of three main components: 
%\textbf{Frozen DINO-X}: We use a frozen DINO-X to extract 
% two-stage features $F^1$ and $F^2$ from the backbone and encoder for region representation based on the input image, and without sacrificing its original excellent localization ability. RoIAlign\cite{he2017mask} operator is employed to extract region features on $F^1$. The region features provide rich detailed information, crucial for OCR and understanding shallow information such as color, material, texture, etc. In particular, the bounding box can also be derived from DINO-X 2 grounding output or external input. 

%\textbf{Object Query Decoder}: constructed from a stack of 6 deformable transformer decoder layers. It takes the image features $F^2$ from the encoder and positional queries $Q^p$ along with content queries $Q^c$ as input and iteratively updates the content queries by interacting with image features. Employing learnable query embeddings to learn versatile object representations has been proven by previous work\cite{carion2020end,zhu2020deformable,li2022dn,liu2022dab,zhang2022dino}, which can provide advanced semantic information. In particular, the positional queries are constructed from normalized bounding box coordinates inspired by\cite{li2022dn,liu2022dab,zhang2022dino}.

%\textbf{Light-weighted Text Decoder}: integrates region features, content queries, along with task tokens to generate response outputs auto-regressively. We adapt OPT-125M~\cite{zhang2022opt} as our text decoder. The learnable task tokens equip the text decoder with the capability of tackling different tasks. 

==> table/pose_estimation/coco_pose.tex <==
\begin{table*}[h]
\centering
\caption{Comparisons with state-of-the-art methods on COCO \texttt{val2017} dataset. $\dag$ denotes the flipping test. $\ddag$ removes the prediction uncertainty estimation in Poseur as a fair regression comparison. The \underline{underlined} highlights the compared results. 
% \emph{Emphasized bold number} in inference time is tested by us, otherwise, from PETR's paper directly or the MMPose official results.
\Revise{The inference time of all methods is tested on an A100, except that the detector of top-down methods is tested by the MMdetection (\textit{i.e.}, $45$ms).}
% The ``RLE'' is a learnable regression-based loss.  
%The \textbf{best results} are highlighted in {\textbf{bold}}.
}
\resizebox{0.9\linewidth}{!}{
  \begin{tabular}{p{0.4cm}l|l|l|l|ccc|cc|c}
    \toprule
       &\multicolumn{2}{c|}{\textbf{Method}} & Backbone & Loss & ${\rm AP}$ & ${\rm AP}_{50}$ & ${\rm AP}_{75}$ & ${\rm AP}_{M}$ & ${\rm AP}_{L}$ & Time [ms]\\
    \midrule
    \parbox{2.5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Two-stage}}}}
    % \multicolumn{10}{c}{\textbf{Two-stage Methods}} \\
    % \midrule
    &\multirow{6}*{{\rotatebox{90}{\textbf{TD}}}}
    & Sim.Base.$^{\dag}$ & ResNet-50 & HM. &70.4 &88.6 & 78.3 & 67.1 & 77.2 & 45$+${{86}}\\
    && HRNet$^{\dag}$ &  HRNet-w32 & HM. & 74.4 & 90.5& 81.9& 70.8& 81.0& 45$+$\Revise{{112}} \\
    &&PRTR$^{\dag}$ & ResNet-50 & R. & 68.2 & 88.2 & 75.2 & 63.2 & 76.2 & 45$+$\Revise{{85}}\\
    &&Poseur &  ResNet-50 & RLE$^{\ddag}$ & 70.0 & - & -&- &- &  45$+${82} \\ 
    &&Poseur &  ResNet-50 & RLE & 74.2 & 89.8 & 81.3&71.1 &80.1 &  45$+${{82}} \\ 
    \cmidrule{2-11}
    &\multirow{3}*{{\rotatebox{90}{\textbf{BU}}}}    
    & HrHRNet$^{\dag}$ &  HRNet-w32 & HM. & 67.1 & 86.2 &73.0 &61.5 &76.1 &  {{322}}\\
    && DEKR$^{\dag}$  &  HRNet-w32 & HM. & 68.0 & 86.7 & 74.5 & 62.1 & 77.7  & -\\
    && SWAHR$^{\dag}$ &  HRNet-w32 & HM. & 68.9 & 87.8 & 74.9 & 63.0 & 77.4 & - \\
        \midrule
    \parbox{2.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{E2E TD}}}}
    %\multicolumn{10}{c}{\textbf{End-to-End Top-down Methods}} \\     
    && Mask R-CNN &  ResNet-101 & HM. &66.0 & 86.9 & 71.5 &- &- & -\\
    &&PRTR$^{\dag}$ & ResNet-101 & HM. & 64.8 &85.1 &70.2& 60.4 &73.8& -\\
    &&Poseur$^{\dag}$ & ResNet-101 & RLE  & 68.6 & 87.5 & 74.8 & - & - & - \\
    &&Poseur$^{\dag}$ & HRNet-w48 & RLE  & 70.1&88.0 & 76.5 & - &- & -\\
    \midrule
    \parbox{2.5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{OS}}}}
    % \multicolumn{10}{c}{\textbf{One-stage Methods}} \\
    % \midrule
    &&InsPose  & ResNet-50 &  R.+HM.  & 65.2& 87.2 & 71.3 & 60.6 & 72.2 & \Revise{78}\\
    &&PETR & ResNet-50 & R.+HM. & 68.8	& 87.5	& 76.3	& 62.7	& 77.7 & {105}  \\
    % &PETR & ResNet-101 &R.+HM. & 70.0 & 88.5	& 77.5 & 63.6 & 79.4 & \underline{123}  \\
    &&PETR & Swin-L & R.+HM.  & 73.1	& 90.7 & 80.9 & 67.2 & 81.7& {206} \\
     \cmidrule{3-11}
    &&ED-Pose\cite{yang2023explicit} & ResNet-50 & R.  &  71.6&  89.6 & 78.1 & 65.9 & 79.8 & 51\\
    % &ED-Pose & ResNet-101 & R.  &   & & & & & \\
    %         % &ED-Pose & ResNet-152 & Reg.  &   & & & & & \\
    &&ED-Pose\cite{yang2023explicit} & Swin-L & R.  &  74.3 & 91.5 & 81.6 & 68.6 & 82.6 & {{88}}  \\
    &&ED-Pose\cite{yang2023explicit} & Swin-L* & R.  &  75.8 & 92.3 & {82.9} & 70.4& 83.5&142 \\
    &&ED-Pose\cite{yang2023explicit} & Swin-L* & R.  &  75.8 & 92.3 & {82.9} & 70.4& 83.5&142 \\
    \midrule


    \parbox{2.5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Ours}}}}
    % \parbox{2.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{DINO-X2}}}}
    &&Frozen DINO-X 2 &enc feat  & R.  &  57.9 & 84.4& 63.3& 54.8& 64.8&- \\
    &&Frozen DINO-X 2 & enc + bb  & R.  &  73.4 & 90.2& 80.2& 68.8 &82.3&- \\
    &&Frozen DINO-X 2 & enc + ladder  & R.  &  75.3 & 91.1& 82.2& 70.6& 83.6&- \\
    &&Trainable DINO-X 2& enc + bb  & R.  &  \textbf{77.8} & \textbf{93.3}& \textbf{83.4}& \textbf{72.1}& \textbf{83.4}&- \\
    &&Frozen DINO-X 2 + aux dataset & enc + bb  & R.  &  74.4 & 90.7& 81.1& 69.3& 83.2&- \\
  \bottomrule
\end{tabular}}
\label{tab:sota}
\vspace{-0.4cm}
\end{table*}

==> table/pose_estimation/crowd_pose.tex <==
\begin{table*}[h]
\vspace{-0.2cm}
  \centering
  \caption{Comparisons with state-of-the-art methods on CrowdPose \texttt{test} dataset. \textbf{TD, BU, OS} mean top-down, bottom-up, and one-stage methods, respectively. We use ``HM.'' and ``R.'' for heatmap-based losses and regression losses. $\dag$ denotes the flipping test. The model with * is pre-trained on Objects365~\citep{ShuaiShao2019Objects365AL} with $5$ feature scales. The \underline{underlined} highlights the compared results. The \textbf{best results} are highlighted in {\textbf{bold}}.}
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lll|l|ccc|ccc}
    \toprule
       &{\textbf{Method}} & backbone & Loss & ${\rm AP}$ & ${\rm AP}_{50}$ & ${\rm AP}_{75}$ & ${\rm AP}_{E}$ & ${\rm AP}_{M}$ & ${\rm AP}_{H}$\\
       \midrule
       %\multicolumn{8}{c}{\textbf{Top-down Methods}} \\
    % \midrule
	\parbox{2.5mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{TD}}}}
    % AlphaPose & - & 61.0 & 81.3 & 66.0 & 71.2 & 61.4 & 51.1  \\
    &Sim.Base & ResNet-50  & HM. & \underline{60.8} & 81.4 & 65.7 & 71.4 &61.2 & 51.2  \\
    &HRNet &HRNet-w48 $\dag$ & HM. & 71.3 & 91.1 & 77.5 & 80.5 & 71.4 & 62.5\\
    &TransPose-H &HRNet-Small-W48 & HM. & 71.8 & 91.5 & 77.8 & 79.5 & 72.9 & 62.2 \\
    &HRFormer-B &HRFormer-B  & HM. & 72.4 & 91.5 & 77.9 & 80.0 & 73.5& 62.4\\
    \midrule
    \parbox{2.5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{BU}}}}
    %\multicolumn{8}{c}{\textbf{ Methods}} \\
    %\midrule
    &HrHRNet-w32 & HrHRNet-w32$\dag$  & HM.  &  65.9  & 86.4 & 70.6 & 73.3 & 66.5 & 57.9\\
    &DEKR & HrHRNet-w32$\dag$ & HM.  & 65.7 & 85.7 & 70.4 & 73.0 & 66.4 & 57.5 \\
    % PINet \TODO{backbone}$\dag$ & HM. & 68.9 &  88.7 & 74.7 & 75.4 & 69.6 & 61.5\\
    &SWAHR & HrHRNet-w32$\dag$& HM. & 71.6 & 88.5 & 77.6 & 78.9 & 72.4 & 63.0\\
    \midrule
    \parbox{2.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{OS}}}}
    % \multicolumn{8}{c}{\textbf{One-stage Methods}} \\
    % \midrule
    &PETR &(Swin-L)  & R.+HM.  & \underline{71.6} & 90.4 & 78.3 & 77.3 & 72.0 & 65.8 \\
       \cmidrule{2-9}
    &ED-Pose\cite{yang2023explicit} & ResNet-50  & R.  &  69.9 & 88.6& 75.8& 77.7& 70.6&60.9 \\
    &ED-Pose\cite{yang2023explicit} &Swin-L  & R.  &  73.1 & 90.5& 79.8& 80.5& 73.8&63.8\ \\
    &ED-Pose\cite{yang2023explicit} &Swin-L* & R.  &  76.6 & \textbf{92.4}& \textbf{83.3}& \textbf{83.0}& \textbf{77.3}& \textbf{68.3} \ \\
    \midrule
    \parbox{2.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Ours}}}}
    &Frozen DINO-X2 & enc feat  & R.  &  63.5 & 85.1& 70.3& -& -&- \\
    &Frozen DINO-X2 & enc + bb  & R.  &  77.1 & 87.3& 82.8& -& -&- \\
    &Frozen DINO-X2 & enc + ladder  & R.  &  \textbf{78.2} & 87.7& 83.2& -& -&- \\
    % &trainable DINO-X2 & enc + ladder  & R.  &  78.2{\color{Red}$\uparrow_{9.1}$} & 87.7& 83.2& -& -&- \\
  \bottomrule
\end{tabular}}
\label{tab:crowdpose}
\vspace{-0.4cm}
\end{table*}

==> table/understanding/dinox-ocr.tex <==
\begin{table}[]
\centering
\resizebox{1\linewidth}{!}{\begin{tabular}{cccccccccccccccccc}
\toprule     
\multirow{2}{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{Regular}}& \multicolumn{6}{c}{\textbf{Irregular}}& \multicolumn{2}{c}{\textbf{Occluded}} & \textbf{Artistic} & \textbf{Handwritten} &  \textbf{Digits} & \multicolumn{2}{c}{\textbf{Semantic}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-10}  \cmidrule(lr){11-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14} \cmidrule(lr){15-15} \cmidrule(lr){16-17}
& IIIT5K & SVT& IC13& IC15& SVTP& CT80& COCO& CTW& TT& HOST& WOST& WordArt& IAM& ORAND& NST& ST\\ 
\midrule
BLIP2-6.7B\cite{li2023blip}& 79.1& 86.7& 83.4& 71.2& 78.8& 76.5& 51.4& 62.4& 68.7& 59.8& 69.4& 68.4& 32.9& 1.2& 13.0& 82.6\\
mPLUG-Owl\cite{ye2023mplug}& 81.1& 84.3& 85.9& 67.5& 73.9& 81.4& 52.3& 69.2& 74.4& 49.7& 62.7& 72.1& 34.8& 13.5& 44.7& 92.3\\
InstructBLIP\cite{panagopoulou2023x}& 86.3& 92.0& 86.8& 80.9& 85.6& 86.3& 62.6& 70.8& 77.9& 67.8& 78.8& 73.7& 42.6& 18.4& 25.3& 89.7\\
LLaVAR\cite{zhang2023llavar}& 84.0& 87.6& 87.7& 79.4& 84.0& 84.5& 61.9& 69.5& 75.6& 61.1& 71.9& 67.1& 49.4& 9.8& 36.2& 86.5\\
BLIVA\cite{hu2024bliva} & 86.5&90.6& 87.3 &80.9& 87.7& 86.7& 64.8& 71.2& 78.1& 67.7& 77.6& 73.7& 45.1& 13.8& 20.4& 89.4\\
mPLUG-Owl2\cite{ye2024mplug}& 80.9& 69.6& 79.8& 53.9& 53.5& 74.8& 52& 59.1& 60.9& 32.5& 50.6& 60.6& 23.8 & 9.9& 48.2& 93.9\\
LLaVA1.5-7B\cite{liu2024visual}& 84.2& 85.7& 86.4& 71.9& 79.8& 82.7& 55.6& 66.8& 73.2& 61.4& 70.6& 68.7& 55.4& 10.4& 15.2& 85.3\\
UniDoc\cite{gu2021unidoc}& 91.9& 89.2& 90.9& 78& 80.3& 88.2& 64.1& 75.3 & 78.2& 52.4& 68.5& -& -& -& -& -\\
Monkey\cite{li2024monkey} & 83.7& 75.1& 85.4& 53.4& 58.4& 73.9& 43.5& 64.5& 64.6& 43.3& 54.9& 67.7& 30.3& 29.1 & 56.5& 95.5\\ \midrule
\rowcolor{blue!5}DINO-X Pro & \multicolumn{1}{c}{74.5} & \multicolumn{1}{c}{81.5} & \multicolumn{1}{c}{86.7} & \multicolumn{1}{c}{66.7} & \multicolumn{1}{c}{73.8} & \multicolumn{1}{c}{79.1} & \multicolumn{1}{c}{41.1} & \multicolumn{1}{c}{61.5} & \multicolumn{1}{c}{56.6} & \multicolumn{1}{c}{41.1} & \multicolumn{1}{c}{53.9} & \multicolumn{1}{c}{54.1} & \multicolumn{1}{c}{40.1} & \multicolumn{1}{c}{10.4} & \multicolumn{1}{c}{38.8} & \multicolumn{1}{c}{86.9} \\ 
\bottomrule
\end{tabular}}
\caption{Results on OCRbench\cite{liu2023hidden}. We report serious accuracy in measuring performance recommended by the paper for evaluation.}
\label{tab:ocr}
\end{table}

==> table/understanding/dinox-vqa.tex <==
\begin{table*}[t!]
\vspace{-.2cm}
    \caption{Results on PointQA local. We report the Exact Match score to evaluate model performance.}
    \label{tab:vqa}
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        Dataset     & BLIP-2~\cite{li2023blip} &  Gemini Pro 1.0~\cite{team2023gemini} & PaLI-X \cite{chen2023pali} & HAMMR-PaLI-X\cite{castrejon2024hammr} & DINO-X Pro \\
        \midrule
        PointQA local & 25.3   & 16.2       & 48.2        & \underline{69.1} & \textbf{70.37}\\
        \bottomrule
    \end{tabular}
    }  %
\end{table*}



